Small-Footprint Open-Vocabulary Keyword Spotting with Quantized LSTM Networks

We explore a keyword-based spoken language understanding system, in which the intent of the user can directly be derived from the detection of a sequence of keywords in the query. In this paper, we focus on an open-vocabulary keyword spotting method, allowing the user to define their own keywords without having to retrain the whole model. We describe the different design choices leading to a fast and small-footprint system, able to run on tiny devices, for any arbitrary set of user-defined keywords, without training data specific to those keywords. The model, based on a quantized long short-term memory (LSTM) neural network, trained with connectionist temporal classification (CTC), weighs less than 500KB. Our approach takes advantage of some properties of the predictions of CTC-trained networks to calibrate the confidence scores and implement a fast detection algorithm. The proposed system outperforms a standard keyword-filler model approach.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> analysis.tex <==
\todo{}

==> appendices.tex <==
% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%
\newpage
\appendices
\section{An experiment on the memory of the CTC-trained LSTMs}
\label{app:lstm-memory}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
\label{app:embedding-perspective}
Appendix two text goes here.

\section{}
Appendix two text goes here.


==> neural.tex <==
As we have seen, the main issue with the previous approach lies in the localized frame prediction. More specifically, it is not trivial to design a confidence score that is both meaningful and discriminative at the keyword level. For CTC-trained acoustic models, we have to deal with the blank predictions, and with such small neural networks, we also have to cope with many confusions or prediction errors at the phone level.

When one knows in advance which keywords the system is designed for, and when one have access to training data containing those keywords, a neural network can be trained to detect the keywords directly, or to give a confidence score at the keyword level (e.g. \todo{cite some}). The idea of the second approach we propose is to generate such a neural network, even for scenarios where the keywords of interest are not known at training time. Basically, at inference, the keywords are given to the system in a configuring step, to generate a neural network the will output keyword-level confidence without retraining the system. To some extent, this approach is similar to other open-vocabulary ASR-free methods \todo{cite them}, except we directly predict the neural network weights from the keywords rather than embeddings fed to the final detection model.


\begin{figure*}[!htb]
    \centering
    \includegraphics[width=\linewidth]{./figs/Model}
    \caption{Overview of the whole model. The first layers of an acoustic model pretrained with CTC serve as an acoustic encoder. The intermediate features are fed to a keyword detector, predicting a detection confidence for each of the keywords. The weights of its last layer (convolutions kernels with size $k$ and $N$ input channels) are predicted by an auxiliary network from the keyword phone sequence.}
    \label{fig:whole_model}
\end{figure*}

The proposed neural network, depicted in Fig.~\ref{fig:whole_model}, has three main components:
\begin{itemize}
    \item an \textbf{acoustic encoder} $AE$, with parameters $\theta^{AE}$, which provides an intermediate representation of the audio signal, suited to ASR
    \item a \textbf{keyword detector} $KD$, with parameters $\theta^{KD}$, which predicts keyword confidence scores from the outputs of the acoustic encoder, and
    \item a \textbf{keyword encoder} $KE$, with parameters $\theta^{KE}$, which predicts the weights of the keyword detector for a given set of keywords.
\end{itemize}

In this section, we will present the components of the neural network, namely the acoustic encoder (Section~\ref{sec:acoustic-encoder}) and keyword encoder and detection (Section~\ref{sec:keyword-detector}). 
We will explain how the network is used for inference in Section~\ref{sec:neural-filters-inference} and how it is trained without keyword-specific data in Section~\ref{sec:neural-filters-training}.
%In Section~\ref{sec:neural-filters-boundaries}, we propose a slight modification to that model allowing to predict the keyword boundaries.
Finally, we discuss advantages and disadvantages of this approach in Section~\ref{sec:neural-filters-proscons}.


\subsection{Acoustic Encoder ($AE$)}
\label{sec:acoustic-encoder}

The acoustic encoder is applied to the input sequence of acoustic feature vectors to produce a sequence of intermediate features vectors $\interm = z_1 \ldots z_{T'(\x)}$ of length $T'(\x)$:

\begin{equation}
    \interm = AE(\x; \theta^{AE})
\end{equation}

As depicted in the left-hand side of Fig.~\ref{fig:whole_model}, the acoustic encoder is the base acoustic model presented in Section~\ref{sec:am} with the last phone classification layer removed. It  is a small stack and skip LSTM network with an initial projection layer, trained with CTC on a large generic speech corpus such as Librispeech to predict the sequence of phonemes from an audio utterance. Although its final performance may be quite poor compared to a state-of-the-art ASR model, the intermediate features it learned while trained to recognize the phones should still be relevant for arbitrary keyword detection.

After training, the last classification layer is removed, and the final intermediate features are fed to the keyword detector. The acoustic encoder, made of all the layers of the base acoustic model except the last one, will not be further trained or fine tuned in the model we present here. Besides simplifying the training procedure, is allows to continue using the acoustic model either for LVCSR or for KWS with the ASR-lite method.




\subsection{Keyword detection}
\label{sec:keyword-detector}

The keyword detector is applied to the sequence of intermediate features vectors $\interm$ to produce a sequence of prediction vectors $\y = y_1 \ldots y_{T''(\x)}$ of length $T''(\x)$:

\begin{equation}
    \y = KD(\interm; \theta^{KD})
\end{equation}
Each vector in the sequence $y_t \in [0,1]^{|\mathcal{K}|}$ contains $|\mathcal{K}|$ coefficients, where $|\mathcal{K}|$ is the number of keywords. The $i$-th coefficient represents the probability of detecting keyword $k_i$ at time $t$.


The keyword detector, depicted in the center illustration of Fig.~\ref{fig:whole_model}, is a two-layer convolutional neural network. From a context window of past intermediate feature frames, it predicts the probability of detection of each keyword in the keyword set at time $t$, i.e. 
\begin{equation}
    y_t = KD(\interm_{t-W:t}; \theta^{KD})
    \label{eq:single-past-detection}
\end{equation}
The first layer aggregates a small context of five frames of intermediate features with a convolution followed by a tanh activation. The obtained representations are pooled and sub-sampled with a max-pooling over three frames every two frames. The last layer is a convolution followed by a sigmoid activation. There is one convolutional kernel for each keyword. Its weights are predicted by a third network: the keyword encoder.

More precisely, the parameters of the keyword detector may be split into a set of shared parameters $\theta^{KD}_{shared}$, corresponding to the weights of the first convolutional layer, and one set of weights $\theta^{KD}_{k_i}$ for each keyword $k_i$, corresponding to the weights of one convolution kernel in the second layer:
\begin{equation}
    \theta^{KD} = \{\theta^{KD}_{shared}\} \cup \bigcup_{k_i \in \mathcal{K}} \theta^{KD}_{k_i}
\end{equation}
Thus $\theta^{KD}_{shared}$ is independent of the set of keywords, and those weights can be determined during training by gradient descent. 
The remaining weights ($\theta^{KD}_{k_i}$) are predicted by an auxiliary neural network.

The keyword encoder (right-hand side of Fig.~\ref{fig:whole_model}) predicts the weights $\theta^{KD}_{k_i}$ of the convolution kernel for the keyword detector from a phone (or character) sequence representation of the keyword $\pseq^{k_i}$: 
\begin{equation}
    \theta^{KD}_{k_i} = KE(\pseq^{k_i}; \theta^{KE})
\end{equation}
In this work, the keyword encoder consists of a bi-directional LSTM layer applied to a sequence of one-hot vector encoding each phone of the keyword, and an affine transform applied to the concatenation of the last output of the LSTM in each direction. The result of this affine transform is interpreted as the weights of the last convolutional layer in the keyword detector. 

Since we apply a threshold on the sigmoid output of the last convolutional layer, we can see the detection as a threshold on the dot product between the concatenation of the kernel weights and the concatenation of its input vectors. We may see the output of the keyword encoder network as an embedding of the keyword. Similarly, the output of the first layer of the keyword detector may be interpreted as an embedding of the audio. Finally, a threshold on the dot product can be reinterpreted as a threshold on the cosine similarity. However, we do not want to frame this problem in an embedding perspective, as we do not necessarily want both representations to lie in a common space. We discuss that topic in more details in Appendix~\ref{app:embedding-perspective}.



\subsection{Inference}
\label{sec:neural-filters-inference}

The inference part may be divided into a configuration step and a detection step.

During the configuration step, the user defines the set of keywords that the model should detect. This step can generally be done offline. 
First, the user provides a set of keywords $\mathcal{K} = \{k_i\}$.
The pronunciation of each keyword ($\pseq^{k_i}$) is retrieved from a lexicon or a grapheme-to-phoneme converter. 
Then the keyword encoder is applied to each keyword pronunciation $\pseq^{k_i}$, to get the weights of the last layer of the keyword detector:
\begin{equation}
    \theta^{KD}_{k_i} = KE(\pseq^{k_i}; \theta^{KE})    
\end{equation}
Finally the parameters of the keyword detector are set to $\theta^{KD} = \{\theta^{KD}_{shared}\} \cup \bigcup_{k_i \in \mathcal{K}} \theta^{KD}_{k_i}$. 

After configuration, the acoustic encoder $AE$ and keyword detector $KD$ jointly make an end-to-end KWS neural network. During the detection step(s), the keyword confidences may be directly predicted from the acoustic features $\x$:
\begin{equation}
    \y = KD(AE(\x; \theta^{AE}); \theta^{KD})
\end{equation}

Keyword detection candidates can be created as in Section~\ref{sec:asr-lite-detection}. However, the start time is unknown. Therefore, most of the post-processor described in Section~\ref{sec:asr-lite-decoding} will not have any effect. The only exception is the ``\textit{greedy with patience}'' one. We will see in Section~\ref{sec:neural-filters-proscons} that with some changes, we can also predict the start time to take advantage of the more elaborated post-processors.

Finally, since the acoustic encoder was designed for easy streaming inference, and since the keyword detector only sees past frames to make a prediction, this model is also compatible with streaming inference.

\subsection{Training}
\label{sec:neural-filters-training}

The inputs of the proposed model are a sequence of acoustic feature vectors $\x$ and one or more phone sequences $\pseq$. These are readily available in any datasets of audio with transcripts such as those used to train a generic acoustic model (e.g. the one of Section~\ref{sec:am}). In generic acoustic model training, the phone sequences are not inputs but serve as supervision for the training. In order to train the proposed model in a supervised manner, we need a target signal for the output $ \y$ of the model. 

Note that the $i$-th component of the output vector at time $t$ should indicate the probability of detecting keyword $k_i$ (or equivalently the phone sequence $\pseq^{k_i}$) at time $t$, i.e.:
\begin{equation}
    y_{t, i} = p(k_i | x_{1:t}, \pseq^{k_i})
    \label{eq:single-past-detection-proba}
\end{equation}
Therefore, if we have an aligned version of the dataset, in which we know at each time step $t$ of the acoustic sequence $\x$, where in the ground-truth phone sequence $\pseq$ we are, we can easily create a training dataset for the proposed model. 

It still holds when the final keywords used at inference time are not present in the training dataset. Basically, since the system is configured with phone sequence, we can generate training samples as follows. 
For each training sample $(\x^{(i)}, \pseq^{(i)}) \in \mathcal{D}$ we create a set of synthetic keywords $\mathcal{K}^{(i)} = {K}^{(i)}_p \cup  \mathcal{K}^{(i)}_n$ containing:
\begin{itemize}
    \item \textit{positive keywords}: $\mathcal{K}^{(i)}_p = \{ k_p \equiv \pi^{(i)}_{n_1} \ldots \pi^{(i)}_{n_2} \}$, with $1 \leq n_1 \leq n_2 \leq |\pi^{(i)}|$, subsequences of $\pseq^{(i)}$ (i.e. occuring in the ground-truth
    \item \textit{negative keywords}: $\mathcal{K}^{(i)}_n = \{ k_n \equiv \tilde{\pi}_{1} \ldots \tilde{\pi}_{M}\}$, with $\tilde{\pi}_{m} \in \mathcal{P}$, not subsequences of $\pseq^{(i)}$ (i.e. not occuring in the ground-truth)
\end{itemize}
We use the alignments create a sequence of supervision vectors 
$\mathbf{v}^{(i)} = v^{(i)}_1 \ldots v^{(i)}_{T'(\x)}$, where $v^{(i)}_t \in \{0, 1\}^{|\mathcal{K}^{(i)}|}$.
Its dimension $|\mathcal{K}^{(i)}|$ corresponds to the number of synthetic keywords. The $k$-th coefficient equals:
\begin{itemize}
    \item $1$ if $k < |\mathcal{K}^{(i)}_p|$ (i.e. one of the positive keywords) and - using the alignments - the $k$-th keyword in $\mathcal{K}_p$ should be detected at time $t$
    \item $0$ otherwise
\end{itemize}
As a result, we have a new dataset $\mathcal{D}' = \{\x^{(i)}, \mathbf{v}^{(i)}, \mathcal{K}^{(i)} \}$, of audio features, synthetic keywords and detection supervision.

For a given training sample $(\x^{(i)}, \mathbf{v}^{(i)}, \mathcal{K}^{(i)})$, the output of the model is computed:
\begin{eqnarray*}
    \interm & = & AE(\x^{(i)}; \theta^{AE}) \\
    \theta^{KD}_k & = & KE(\pseq^{k}; \theta^{KE}),~~~\forall k \in \mathcal{K}^{(i)} \\
    \y & = & KD(\interm; \{\theta^{KD}_{shared}\} \cup \bigcup_{k \in \mathcal{K}^{(i)}} \theta^{KD}_{k}) \\ 
\end{eqnarray*}
and we can compute the cross-entropy loss:
\begin{equation}
    l(i) = - \sum_{d=1}^{|\mathcal{K}^{(i)}|} \sum_{t=1}^{T''(\x)} v_{t,d}^{(i)}\ln y_{t,d} + (1-v_{t,d}^{(i)})\ln(1 - y_{t,d})
\end{equation}

The keyword detector and encoder are jointly trained to determine the parameters $\theta^{KE}, \theta^{KD}_{shared}$ by minimizing the loss on the whole dataset:
\begin{equation}
    \theta^{KE}, \theta_{shared}^{KD} = \arg\min \sum_{\{\x^{(i)}, \mathbf{v}^{(i)}, \mathcal{K}^{(i)}\} \in \mathcal{D'}} l(i)
\end{equation}
The parameters of the acoustic encoder were already trained during the base acoustic model training, and remain fixed, as mentioned in Section~\ref{sec:acoustic-encoder}.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{./figs/TrainingSample.png}
    \caption{Traning sample creation. The blue stripes represent the intermediate feature frames ($\interm$). The squares below represent the aligments (\texttt{-} representing the \textit{blank} label). At a given time step (red rectangle) we extract a context of $W$ past frames and $N$ last phones.
    \label{fig:training-sample}}
\end{figure}

In practice, we can take advantage from using mini-batches during training and from the acoustic encoder not being fine-tuned to simplify the process. The acoustic encoder is not trained here so we first extract its outputs:
\begin{equation}
    \interm^{(i)} = AE(\x^{(i)}; \theta^{AE})
\end{equation}
To predict $y_t$ the keyword detector will only see a limited context corresponding to the size of its receptive field $W$. 
At every time step of a given utterance, we extract a window of $W$ past frames, and a sequence of the last $N$ ground-truth phone at this time step, as shown on Fig.~\ref{fig:training-sample}. The synthetic keywords will be created from these last $N$ phones. We set $N$ to the maximum keyword length that we want to support (e.g. $10$). Since we do not fine-tune the acoustic encoder, the fast that the last $N$ phone are not included in the window of $W$ frames might be problematic. We discuss that issue in Appendix~\ref{app:lstm-memory}.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{./figs/Training.png}
    \caption{Mini-batch creation for the training of the generic keyword spotting model (here, $K=|\mathcal{K}_p|=2$ and $B=4$).}
    \label{fig:training}
\end{figure}

During training, we create batches of $B$ samples. For each sample, we create $|\mathcal{K}_p|$ synthetic (positive) keywords. Each keyword is a suffix of the extracted phone sequence, with a length uniformly sampled between $3$ and $N$. The negative keywords $\mathcal{K}_n$ for a given sample will be the positive keywords of the other samples in the batch.
In general, there will be $|\mathcal{K}_p|$ positive keywords, and $|\mathcal{K}_p|(B-1)$ negative ones for each training sample in the batch.

The $K \times B$ keywords are fed to the keyword encoder, which predicts the $K \times B$ kernels of the last convolution layer, for each synthetic keyword. The obtained keyword detector is applied to the $B$ acoustic samples of $W$ frames each. It results in $K \times B$ prediction outputs for each of the $B$ samples. 
The network is trained with a cross-entropy loss, to predict $1$ for the keywords that match a suffix of the $N$ phones extracted for the samples, and $0$ everywhere else. The process is illustrated in Fig.~\ref{fig:training}.


\subsection{Advantages of this approach}
\label{sec:neural-filters-proscons}

This end-to-end approach has some advantages and disadvantages compared to the ASR-lite method. We list some of them here.

\subsubsection{Discriminative at the keyword level} This model directly outputs a confidence score for the whole keyword, alleviating the need of confidence score calibration. The level of confusion is also reduced as the keywords tend to either be detected with high confidence of not detected at all.

\subsubsection{Easier to fine-tune when specific training data is available} Since the ASR-lite method relies on phone predictions, it would not take so much advantage of the availability of specific training data (containing the keywords). With the neural filter method, the parameters predicted by the keyword encoder could serve as an initialization of the top convolutional layer. These parameters could be fine-tuned on keyword-specific training data, and could be helpful in small dataset regimes.

\subsubsection{May learn from acoustic model confusions} The base acoustic model is small and makes many prediction errors (over 20\% on clean audio). The ASR-lite method may suffer from phone prediction errors because each phone contributes individually to the final detection. In the neural filters method, the detector is trained on top of the base acoustic model and may learn from its confusions. 

\subsubsection{Predictability of confusions}
Keywords with similar convolution kernels will have similar confidence score for a given input. Thus the output of the keyword encoder may give us a proxy to analyse what the model learns, or how it will behave for a given keyword set. 

\subsubsection{Prediction of keyword boundaries}
\label{sec:neural-filters-boundaries}
The model we have presented detects keywords as soon as the finish. Therefore we know the end of the keyword but not its start, preventing the application of the ``sequence'' post-processor presented in Section~\ref{sec:asr-lite-decoding}. Yet it only comes from how the problem was framed. The same model can be seen symmetrically and made to predict the beginning of a keyword after a delay of $W$ frames. If we rewrite equations~\ref{eq:single-past-detection} and~\ref{eq:single-past-detection-proba} as:
\begin{eqnarray*}
    y_t & = & KD(\interm_{t:t+W}; \theta^{KD}) \\
    y_{t, i} & = & p(k_i | x_{t:t+W}, \pseq^{k_i})
\end{eqnarray*}
and build the dataset from the alignments accordingly, the exact same model will be trained to detect the beginning of keywords. 
Moreover, we may train one keyword encoder to predict the parameters to detect the start of a keyword, and a second encoder to predict the parameters allowing to detect the end. Using both predictions, we can create detection candidates, e.g. multiplying the confidence of start at some time $t_s$ by that of end at time $t_e$. This enables the use of more elaborated post-processors like the sequence one.

\subsubsection{Harder to tweak and interpret}
Like many end-to-end models, how the model predicts a keyword (or fails to) is harder to interpret and understand. In the phone-based ASR-lite method, one can look at the predictions of the neural network and have a better understanding of why a keyword was not predicted. This allows to design methods to tweak the system, as done for example in~\cite{lugosch2018donut,yang2018automatic}. It is not possible, or more difficult to do with the end-to-end model.

\subsubsection{Less scalable}
Whereas in the ASR-lite method, the neural network will always have the same size whatever the number of keywords, for this one, the number of parameters grow linearly with the size of the keyword set.

==> sota.tex <==
\todo{rewrite literature review}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{./figs/neural_kws}
    \caption{Neural approaches to keyword spotting keyword spotting. Left: direct keyword spotting, the neural network predicts a detection score for each keyword (usually requires specific training data). Right: ASR-based approach, the network predicts phone sequences that need to be post-processed (common approach to open-vocabulary KWS).\label{fig:neural_kws}}
\end{figure}




A significant amount of work has been proposed to classify speech commands  in a predefined set or to detect wakewords with tiny neural networks under 500KB~\cite{sainath2015convolutional,coucke2019efficient}. However, these methods require specific training data, and are not suited to scenarios where training data is not readily available. Keyword spotting methods may be divided into two categories: query-by-example scenarios where the system is configured with example audios of the keywords, or query-by-string, where the system is configured by typing keywords. We are interested in the second type. Query-by-string scenarios can be further divided into ASR-based systems in which the keyword is detected from a transcription of the audio into words, characters or phones, or ASR-free systems which directly perform the detection from intermediate representations of the audio input and keywords, without relying on the transcription. Our model belongs to the latter category.  

Traditional ASR-based keyword spotting approaches consist in building models for keywords and ``background" and computing likelihood ratios between the two~\cite{szoke2005comparison}.
More recently, new approaches based on end-to-end neural speech recognition systems trained to predict phone sequences emerged.
%More recently, with end-to-end acoustic neural network predicting phone sequences, for example trained with CTC~\cite{graves2006connectionist}, new approaches emerged to 
They look for the keyword phone sequence in the network predictions, for example by trying to match the keywords in predicted phones lattices~\cite{chen2017confidence} or from the transcription directly, taking into account the confusions of the network~\cite{lugosch2018donut,yang2018automatic}.

ASR-free approaches generally consist in computing embeddings for both the audio and the keyword pronunciation~\cite{audhkhasi2017end,sacchi2019open}. In~\cite{audhkhasi2017end}, the whole spoken utterance is embedded into a single vector with a recurrent auto-encoder. Similarly, the keyword is embedded into a vector using an auto-encoder of the phone sequence. The concatenation of both vectors is fed to a small neural network predicting whether the keyword appears in the utterance. In~\cite{sacchi2019open}, different recurrent neural networks are trained to predict the word and phone embeddings. The classification is based on the distance between the keyword and utterance embedding. This method seems to be only applicable to isolated words and cannot handle keywords in a natural language utterance.
%
%The last two models require access to audio-phone alignments obtained with an ASR but do not pretrain the acoustic embeddings with an ASR criterion. We argue that even if the resulting acoustic model would be poor, it would still learn features that would be relevant for keyword spotting.

In the model we propose, a recurrent neural network is applied to the keyword pronunciations to predict the weights of the topmost convolution kernel of the keyword detector network. This idea is similar to other works on dynamic convolution filters in computer vision for weather prediction~\cite{klein2015dynamic}, visual question answering~\cite{noh2016image}, or video and stereo prediction~\cite{jia2016dynamic}.


